Improving Reliability, Security, and Efficiency of Reconfigurable Hardware Systems

In this treatise, my research on methods to improve efficiency, reliability, and security of reconfigurable hardware systems, i.e., FPGAs, through partial dynamic reconfiguration is outlined. The efficiency of reconfigurable systems can be improved by loading optimized data paths on-the-fly on an FPGA fabric. This technique was applied to the acceleration of SQL queries for large database applications as well as for image and signal processing applications. The focus was not only on performance improvements and resource efficiency, but also the energy efficiency has been significantly improved. In the area of reliability, countermeasures against radiation-induced faults and aging effects for long mission times were investigated and applied to SRAM-FPGA-based satellite systems. Finally, to increase the security of cryptographic FPGA-based implementations against physical attacks, i.e., side-channel and fault injection analysis as well as reverse engineering, it is proposed to transform static circuit structures into dynamic ones by applying dynamic partial reconfiguration.

==> bib.tex <==
\chapter{Bibliography}


\nocite{patep,patus}
\nocite{ZBB16,WRZT:2013,ZT09,ZT07,KHZ16,HKZ15,HKZ14,zie10,KZH16,zst10,EWBTZ16, PZ6, BEZWT:2016, BZMT15,BEZT15,GRBZFTH15,DBLP:conf/fpl/Becher14, RAW:2014, FCCM:2014, Schmidt:2014:ANF:2554688.2554730, SZT14,FCCM:2013,  ZBTZ12,GYRT2012, FCCM:2012, KZF12,DBLP:conf/fpt/AngermeierZGT11,DBLP:conf/codes/WildermannRZT11,DBLP:conf/fpl/AngermeierZGT11, DBLP:conf/fpl/WildermannTZ11, ZWOWT11, TZ11, ZT10,ZBT10b, ZBT10,
 MBZ10,SZT2008,ZT2008, AISEC2007, AIS2007, ZT2006, ZAT2006,AHWZ06, DBLP:conf/fpt/ZiermannSMZAT11,AIS2009,ZT05}

\section{General Bibliography}
\newrefcontext[sorting=nyt]
\printbibliography[notcategory=patents,notcategory=journals,notcategory=books,notcategory=bookchapters,notcategory=conferences,notcategory=miscs,heading=subbibliography,title={General Bibliography},heading=none]


% 
% %\bibliographystyle{alpha}
% \begingroup
% 
% \renewcommand{\refname}{}
% %\renewcommand{\section}[2]{}%
% \renewcommand{\chapter}[4]{} % for other classes
% 
% 
% %
% 
% \bibliographystyle{plain} 
% 
% 
% \bibliography{bibentries,literature,literature_FSP}
% \endgroup
 \cleardoublepage

\section{Personal Bibliography}\label{sec:mypup}

\let\etalchar\undefined % undefine \etalchar defined by previous bibliography
%\renewcommand{\refname}{Author's Own Publications}
%\bibliographystyleme{alpha}
%\nociteme{opt4j}
%\bibliographyme{me}


Note that the publications included in this cumulative treatise in Appendix B are highlighted with blue color. 

\subsubsection{Awards:}

\begin{tabbing}
\hspace{2cm} \= \hspace{7cm} \= \kill
\>Best Paper Award: \> FPT 2006, ReConFig 2016 \\
\>Best Application Paper Award: \> AHS 2015 \\
\>Best Paper Candidate: \> CODES+ISSS 2011 \\ 
\end{tabbing}

\subsubsection{Patents:}
\newrefcontext[labelprefix=P]
\printbibliography[category=patents,resetnumbers,heading=none]
 
% 

%  
% 
% 
% \nociteP{patep}
% \nociteP{patus}
% %\vspace{-20 mm}
% 
% \begingroup
% 
% \renewcommand{\refnameP}{}
% %\renewcommand{\section}[2]{}%
% \renewcommand{\chapter}[4]{} % for other classes
% 
% 
% \bibliographystyleP{plainyr-rev}
%  %hundreds of styles to choose from
% \bibliographyP{ziener}
% 
% \endgroup
% 
\subsubsection{Books:}


\newrefcontext[labelprefix=B]
%\newrefcontext[sorting=dynt]
\printbibliography[sorting=ydnt,category=books,resetnumbers,heading=none]



% 
% \nociteB{KHZ16}
% \nociteB{HKZ15}
% \nociteB{HKZ14}
% \nociteB{zie10}
% %\vspace{-20 mm}
% \begingroup
% \renewcommand{\refnameB}{}
% \renewcommand{\chapter}[4]{}
% \bibliographystyleB{plainyr-rev} %hundreds of styles to choose from
% \bibliographyB{ziener}
% 
% \endgroup
% 
\subsubsection{Book Chapters:}

\newrefcontext[labelprefix=BC]
%\newrefcontext[sorting=dynt]
\printbibliography[sorting=ydnt,category=bookchapters,resetnumbers,heading=none]

% 
% \nociteBC{KZH16,zst10}
% %\vspace{-20 mm}
% \begingroup
% \renewcommand{\refnameBC}{}
% \renewcommand{\chapter}[4]{}
% \bibliographystyleBC{plainyr-rev} %hundreds of styles to choose from
% \bibliographyBC{ziener}
% \endgroup
% %\newpage
\subsubsection{Journals:}

\newrefcontext[labelprefix=J]
%\newrefcontext[sorting=dynt]
\printbibliography[sorting=ydnt,category=journals,resetnumbers,heading=none]
 

% 
% \nociteJ{ZBB16,WRZT:2013,ZT09,ZT07}
% %\vspace{-20 mm}
% \begingroup
% \renewcommand{\refnameJ}{}
% \renewcommand{\chapter}[4]{}
% \bibliographystyleJ{plainyr-rev} %hundreds of styles to choose from
% \bibliographyJ{ziener}
% \endgroup

% 
\subsubsection{Conferences: (peer reviewed)}


\newrefcontext[labelprefix=C,sorting=ydnt]
%\newrefcontext[sorting=ydnt]
\printbibliography[category=conferences,resetnumbers,heading=none]
 


% 
% 
% 
% \nociteC{EWBTZ16, PZ6, BEZWT:2016, BZMT15,BEZT15,GRBZFTH15,DBLP:conf/fpl/Becher14, RAW:2014, FCCM:2014, Schmidt:2014:ANF:2554688.2554730, SZT14,FCCM:2013,  ZBTZ12,GYRT2012, FCCM:2012, KZF12,
% DBLP:conf/fpt/AngermeierZGT11,DBLP:conf/codes/WildermannRZT11,DBLP:conf/fpl/AngermeierZGT11, DBLP:conf/fpl/WildermannTZ11, ZWOWT11, TZ11, ZT10,ZBT10b, ZBT10,
%  MBZ10,SZT2008,ZT2008, AISEC2007, AIS2007, ZT2006, ZAT2006,AHWZ06}
% %\vspace{-20 mm}
% \begingroup
% \renewcommand{\refnameC}{}
% \renewcommand{\chapter}[4]{}
% \bibliographystyleC{plainyr-rev} %hundreds of styles to choose from
% \bibliographyC{ziener}
% \endgroup
%  
% %\newpage
 \subsubsection{Miscs:}
 
 \newrefcontext[labelprefix=M]
%\newrefcontext[sorting=dynt]
\printbibliography[sorting=ydnt,category=miscs,resetnumbers,heading=none]
 

 
% 
% \nociteM{DBLP:conf/fpt/ZiermannSMZAT11,AIS2009,ZT05}
% %\vspace{-20 mm}
% \begingroup
% \renewcommand{\refnameM}{}
% \renewcommand{\chapter}[4]{}
% \bibliographystyleM{plainyr-rev} %hundreds of styles to choose from
% \bibliographyM{ziener}
% \endgroup
%  

\chapter{Paper Reprints}\label{sec:mainpapers}


This document is a cumulative habilitation treatise. I have selected out of my 45 peer-reviewed publications, listed in Appendix \ref{sec:mypup}, the following seven papers as the key contributions of my research. 

\vspace{0.5cm}

\noindent \textbf{Methods for Improving the Efficiency of Reconfigurable Systems:}

\vspace{-2mm}

\renewcommand{\arraystretch}{3.6}
\begin{tabular}{l l l} 
\textbf{FCCM'12} & \pbox{10cm}{\small Christopher Dennl, Daniel Ziener, and J{\"u}rgen Teich.  \emph{On-the-fly Composition of FPGA-Based SQL Query Accelerators Using A Partially Reconfigurable Module Library}} & \cite{FCCM:2012} \\
\textbf{FPL'14} & \pbox{10cm}{\small Andreas Becher, Florian Bauer, Daniel Ziener, and J{\"u}rgen Teich.  \emph{Energy-Aware SQL Query Acceleration through FPGA-Based Dynamic Partial Reconfiguration.}} & \cite{DBLP:conf/fpl/Becher14} \\
\textbf{FPT'15} & \pbox{10cm}{\small Andreas Becher, Daniel Ziener, Klaus Meyer-Wegener, and J{\"u}rgen Teich.   \emph{A Co-Design Approach for Accelerated SQL Query Processing via FPGA-based Data Filtering}} & \cite{BZMT15} \\
\textbf{TRETS'16} & \pbox{10cm}{\small Daniel Ziener, Florian Bauer, Andreas Becher, Christopher Dennl, Klaus Meyer-Wegener, Ute Sch{\"u}rfeld, J{\"u}rgen Teich, J{\"o}rg-Stephan Vogt, and Helmut Weber.  \emph{FPGA-Based Dynamically Reconfigurable SQL Query Processing}} & \cite{ZBB16} \\
\end{tabular}

\vspace{0.5cm}

\noindent \textbf{Methods for Improving the Reliability of Reconfigurable Systems:}
\vspace{-2mm}

\begin{tabular}{l l l} 

\textbf{FPT'11} & \pbox{10cm}{\small Josef Angermeier, Daniel Ziener, Michael Gla{\ss},  and J{\"u}rgen Teich.  \emph{Runtime Stress-aware Replica Placement on Reconfigurable Devices under Safety Constraints}} & \cite{DBLP:conf/fpt/AngermeierZGT11} \\
\textbf{FCCM'14} & \pbox{10cm}{\small Robert Glein, Bernhard Schmidt, Florian Rittner, J{\"u}rgen Teich, and Daniel Ziener.  \emph{A Self-Adaptive SEU Mitigation System for FPGAs with an Internal Block RAM Radiation Particle Sensor}} & \cite{FCCM:2014} \\
\textbf{AHS'15} & \pbox{10cm}{\small Robert Glein, Florian Rittner, Andreas Becher, Daniel Ziener, J{\"u}rgen Frickel, J{\"u}rgen Teich, and Albert Heuberger. \emph{Reliability of Space-Grade vs. COTS SRAM-Based FPGA in N-Modular Redundancy}} & \cite{GRBZFTH15} \\

\end{tabular}


\section{On-the-fly Composition of FPGA-Based SQL Query Accelerators Using A Partially Reconfigurable Module Library}

\cite{FCCM:2012} Proceedings of the IEEE International Field-Programmable Custom Computing Machines Symposium (FCCM), 2012 

\includepdf[pages=-]{papers/06239790.pdf}

\section[Energy-Aware SQL Query Acceleration through FPGA-Based Dynamic Partial Reconfiguration]{Energy-Aware SQL Query Acceleration through FPGA-Based Dynamic Partial Reconfiguration%
\sectionmark{Energy-Aware SQL Query Acceleration through FPGA-Based DPR}}
\sectionmark{Energy-Aware SQL Query Acceleration through FPGA-Based DPR}

\cite{DBLP:conf/fpl/Becher14} Proceedings of the International Conference on Field Programmable Logic and Applications (FPL), 2014 


\includepdf[pages=-]{papers/06927502.pdf}


\section{A Co-Design Approach for Accelerated SQL Query Processing via FPGA-based Data Filtering}

\cite{BZMT15} Proceedings of the IEEE International Field-Programmable Custom Computing Machines Symposium (FCCM), 2015  



\includepdf[pages=-]{papers/07393148.pdf}


\section{FPGA-Based Dynamically Reconfigurable SQL Query Processing}



\cite{ZBB16} ACM Transactions on Reconfigurable Technology and Systems (TRETS), 2016 

\includepdf[pages=-]{papers/a25-ziener.pdf}


\section{Runtime Stress-aware Replica Placement on Reconfigurable Devices under Safety Constraints}

\cite{DBLP:conf/fpt/AngermeierZGT11} Proceedings of the International Conference on Field-Programmable Technology (FPT), 2011 



\includepdf[pages=-]{papers/06133247.pdf}

\section[A Self-Adaptive SEU Mitigation System for FPGAs with an Internal Block RAM Radiation Particle Sensor]{A Self-Adaptive SEU Mitigation System for FPGAs with an Internal Block RAM Radiation Particle Sensor%
\sectionmark{A Self-Adaptive SEU Mitigation System for FPGAs}}


\cite{FCCM:2014} Proceedings of the IEEE International Field-Programmable Custom Computing Machines Symposium (FCCM), 2014 


\includepdf[pages=-]{papers/06861641.pdf}

\section{Reliability of Space-Grade vs. COTS SRAM-Based FPGA in N-Modular Redundancy}


\cite{GRBZFTH15} Proceedings of 2015 NASA/ESA Conference on Adaptive Hardware and Systems (AHS), 2015


\includepdf[pages=-]{papers/07231159.pdf}




